MobILE: Model-Based Imitation Learning From Observation Alone

This paper studies Imitation Learning from Observations alone (ILFO) where the learner is presented with expert demonstrations that consist only of states visited by an expert (without access to actions taken by the expert). We present a provably efficient model-based framework MobILE to solve the ILFO problem. MobILE involves carefully trading off strategic exploration against imitation - this is achieved by integrating the idea of optimism in the face of uncertainty into the distribution matching imitation learning (IL) framework. We provide a unified analysis for MobILE, and demonstrate that MobILE enjoys strong performance guarantees for classes of MDP dynamics that satisfy certain well studied notions of structural complexity. We also show that the ILFO problem is strictly harder than the standard IL problem by presenting an exponential sample complexity separation between IL and ILFO. We complement these theoretical results with experimental simulations on benchmark OpenAI Gym tasks that indicate the efficacy of MobILE. Code for implementing the MobILE framework is available at https://github.com/rahulkidambi/MobILE-NeurIPS2021.

==> docs/exp.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-CartPole-v1-3.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-CartPole-v1-5.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-CartPole-v1-10.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-CartPole-v1-20.pdf}
    \end{subfigure}\\
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Reacher-v2-5.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Reacher-v2-10.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Reacher-v2-20.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Reacher-v2-40.pdf}
    \end{subfigure}\\
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Swimmer-v4-5.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Swimmer-v4-10.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Swimmer-v4-20.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Swimmer-v4-40.pdf}
    \end{subfigure}\\
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Hopper-v6-5.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Hopper-v6-10.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Hopper-v6-20.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/Returns-Hopper-v6-40.pdf}
    \end{subfigure}\\
    \caption{%\scriptsize 
    Comparing~\algname~(red) against BC (green) and Expert (blue) on~\cartpole~($1^{\text{st}}$ row), \reacher~($2^{\text{nd}}$ row), \swimmer~($3^{\text{rd}}$ row), \hopper~($4^{\text{th}}$ row)~with four different amounts of expert trajectories. \algname~matches or exceeds the performance of BC across these benchmark tasks despite BC having access to expert actions and \algname~working without expert actions.}\label{fig:performance}
\end{figure*}
% ============================
% ======= Experiments ========
% ============================
\vspace{-3mm}
\section{Experiments}
\vspace{-2mm}
\label{sec:exp}
This section seeks to answer the following questions:
\begin{itemize}[leftmargin=*]
    \item {\bf\algname's empirical performance:} How does \algname{} perform relative to other model-based methods for ILFO?
    \item {\bf Importance of optimism:} Is optimism important for solving ILFO with~\algname? How does~\algname~behave with varying levels of optimism?
    \item {\bf Behavior in stochastic environments:} How does \algname{} perform in MDPs with stochastic dynamics?
\end{itemize}
We consider benchmark tasks from Open AI Gym~\citep{brockman2016openai} simulated with Mujoco~\citep{todorov2012mujoco}. We evaluate \algname{} in \cartpole, \reacher, \swimmer, and \hopper. For \reacher~and \swimmer, following \citep{Sun19FAIL}, we discretize every action dimension into five equally spaced bins between the minimum and the maximum value. For \hopper, we work with continuous actions. We train an expert for each task using TRPO \citep{SchulmanTRPO} until the expert hits an average value of $460, -10, 38, 3000$ for \cartpole, \reacher, \swimmer, \hopper{} respectively. We setup \swimmer, \hopper{} similar to prior model-based RL works~\citep{KurutachCDTA18,nagabandi2018neural,luo2018algorithmic,RajeswaranGameMBRL}. We report results with $3, 5, 10, 20$ expert trajectories for \cartpole{} and with $5, 10, 20, 40$ expert trajectories for \reacher, \swimmer, \hopper. All results are averaged over $3$ seeds.\\
\begin{figure*}[ht]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/True-Reward-Ablations-Reacher-v2-10.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/IntrinsicReward-Reacher-v2-10.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/True-Reward-Ablations-Hopper-v6-10.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=0.24\textwidth]{figures/IntrinsicReward-Hopper-v6-10.pdf}
    \end{subfigure}
    \caption{From left to right: first/third plot -- learning curves (without error bars to avoid clutter) with varying $\lambda$ for \reacher,~\hopper; second/fourth plot --
    plot of bonus as a function of algorithm progress for best value of $\lambda$ for \reacher,~\hopper. 
    %the first and third plots show learning curves for Reacher-v2 and Hopper-v2 with various $\lambda$ values, and the second and fourth plots show the bonus values for Reacher-v2 and Hopper-v2 throughout learning respectively. Comparing the effect of bonus strength $\lambda$ on the performance of ~\algname. 
    Higher $\lambda$ implies larger bonuses added to the rewards. Note that lower values of $\lambda$ leads to slow (sample inefficient) learning, while, higher $\lambda$ also lead to highly sub-optimal behavior. Successful imitation requires trading off exploration and imitation with intermediate values of $\lambda$.}\label{fig:bonus}
\end{figure*}

\noindent In terms of benchmarks, we compare \algname~against BC instead of other model-based ILFO algorithms because: (a) BC in principle upper-bounds the performance of approaches such as BC-O~\citep{TorabiBCO} (this is also observed in the empirical results reported from \cite{TorabiBCO}); (b) other approaches like \citep{EdwardsILPO} require discrete actions, whereas, \algname~works with and is benchmarked in environments with continuous actions. Furthermore, note that BC is a non-trivial benchmark compared to other ILFO approaches since \emph{it has access to expert actions}. Note that \algname~does not have access to expert actions. Furthermore, we run BC with three different seeds and take the best performing policy from each of the three runs, even if they occur at different iterations and report the average of these numbers. More details of experimental setup is discussed in Appendix~\ref{sec:implementation_details}. As we will show, with reasonable amount of optimization and parameter tuning, BC actually can serve as a very strong baseline and nearly solves \emph{deterministic} Mujoco environments, which is indeed consistent to the observations from prior \citep{brantley2020dril} and recent work \citep{spencer2021feedback} in IL.

\subsection{Benchmarking~\algname~on MuJoCo suite}\label{ssec:expt_benchmark} Figure~\ref{fig:performance} presents a comparison of \algname~with BC. Note that \algname~matches or exceeds BC's performance \emph{despite BC having access to actions taken by the expert} and \algname~functioning {\em without} expert action information. This indicates that \algname~improves upon the performance of BC-O~\citep{TorabiBCO}, since it tends to be outperformed by BC. Moreover, we see that BC offers strong performance in these benchmarks owing to determinism in the transition dynamics; we return to this issue in section~\ref{ssec:expt_stochastic}, where we compare \algname~with BC on environments that exhibit stochastic transition dynamics.

\subsection{Importance of the optimistic MDP construction}\label{ssec:expt_ablation}
We consider two environment/expert trajectory combinations namely, \reacher~and \hopper~with $10$ expert trajectories. We vary the amount of exploration performed by \algname~by varying $\lambda$ (the weight of the bonus). Figure~\ref{fig:bonus} indicates that the value of $\lambda$ does tend to influence the performance of \algname. In particular, $\lambda=0$ implies the algorithm is not {\em explicitly} incentivized to explore; it can still explore because of randomness in actions when sampling from the stochastic policy. We observe that the regime with lower $\lambda$ is typically associated with sample inefficiency in terms of number of online interactions needed to solve the problem. Alternatively, a large $\lambda$ implies the algorithm tends to over-explore and is not adequately rewarded for distribution matching. The key to the success of \algname~is to balance exploration with imitation. Empirically, we tend to observe an initial increase in the bonus signifying that the algorithm explores followed by a decay as the algorithm trades-off exploration for successful imitation.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/Returns-CartPole-v2-100.pdf}
    \caption{\algname{} benchmarked against BC in a stochastic variant of \cartpoles. While BC (in green color) struggles with stochastic transition dynamics, note that \algname~(in red color) performs reliably even in this harder setting.}
    \label{fig:stochastic}
\end{figure}

\subsection{Performance with stochastic environments}\label{ssec:expt_stochastic}
\noindent This section considers a stochastic variant of \cartpoles, wherein, additive Gaussian noise with zero mean is added to the transition dynamics. The variance of the additive Gaussian noise is not known to the learner. Figure~\ref{fig:stochastic} presents the results of BC in comparison to \algname~for this problem. Figure~\ref{fig:stochastic} indicates that even this minor modification to the transition dynamics of the environment (to make it stochastic) leads to rapid degradation of BC's performance. This result indicates that stochastic transition dynamics are not straightforward for algorithms relying on BC, for e.g., BC-O to reliably solve. In contrast, \algname~successfully solves the ILFO problem even for environments with stochastic transition dynamics.

==> docs/prelim.tex <==
\section{Preliminaries}


==> docs/rmax.tex <==
\newcommand{\sa}{(s,a)}
%\newcommand{\proj}

\section{Setting}

\subsection{MDPs}

%Definition of Bellman Completeness and linear closure. 
Given any function $f:\Scal\times\Acal \to \mathbb{R}$, denote Bellman operator $\Tcal_h f: \Scal\times\Acal\to\mathbb{R}$ as $\Tcal_h f\sa := r_h\sa + \EE_{s'\sim P_h(\cdot|s,a) }\left[\max_{a'\in\Acal} f(s',a')\right]$.

\subsection{Bellman Completeness}

Given a feature representation $\phi: \Scal\times\Acal \to \mathbb{R}^d$ with $\sup_{\sa} \|\phi\sa\|_2\leq 1$. Given any weight vector $\theta\in \mathbb{R}^d$, we denote $\theta\cdot \phi : \Scal\times\Acal\to\mathbb{R}$ as a mapping $\theta\cdot\phi\sa$ that maps from state-action pair $\sa$ to a scalar. We define Bellman completeness as follows. 
\begin{definition}[Bellman Completeness] There exists a sequence of balls $\Bcal_h = \{\theta: \|\theta\|_2\leq W_h\}$ for all $h\in [H]$ such that, at any $h\in [H]$, given any reward $r_h\sa = \theta\cdot\phi\sa$ with $\|\theta\|_2\leq 1$, and $\theta'$ with $\|\theta'\|_2\in \Bcal_{h+1}$, there exists a vector $\widetilde{\theta}\in\Bcal_h$, such that $\widetilde{\theta}\cdot \phi\sa = \theta\cdot\phi\sa + \EE_{s'\sim P_h(\cdot|s,a)}\left[\max_{a' } \theta'\cdot \phi(s',a')\right]$ for all $\sa\in\Scal\times\Acal$.
%Starting with any $\theta_{H} $ with $\|\theta \|_{2} \leq W$, we have that for any $h$, there exists $\theta_h$ with $\|\theta_h \|_2\leq W$ such that $\theta_h\cdot \phi\sa = \Tcal_h \left(\theta_{h+1}\cdot \phi\right)\sa$.
\label{def:bellman_complete}
\end{definition}
\wen{this def needs to be refined...}

The above definition says that at any time step $h$, given some reward $r_h$ that linear in the feature space $\phi$, and a function $f$ that is linear in $\phi$ as well, then applying Bellman operator $\Tcal_h$ using $r_h$ on $f$ resulting another linear function that is linear in the feature space $\phi$.

\begin{proposition}
Bellman Completeness captures both Linear Quadratic Regulator and Linear MDPs.
\end{proposition}



\section{Algorithm}

The algorithm is described in~\pref{alg:rmax}. For any time step $h$, we maintain a set of policies $\Pi_h$ where any $\boldpi\in \Pi_h$ is a non-stationary policy whose length is $h-1$, i.e., $\boldpi_h = \{\pi_1,\dots, \pi_{h-1}\}$and we denote $d_h^{\boldpi}$ as the state-action distribution induced by $\boldpi$ at time step $h$. Such a policy set $\Pi_h$ provides a mixture distribution $\rho_h = \sum_{\pi\in \Pi_h} d_h^\pi / |\Pi_h| $, which will be used as the restart distribution for FQI subroutines. Sampling a state-action pair from $\rho_h$ can be done by first uniformly sampling a policy from $\Pi_h$, and then executing the selected policy to time step $h$ to get $(s_h,a_h)$.

We denote $\Sigma_h$ as the uncentered covariance matrix $\EE_{\sa\sim \rho_{h}}\phi\sa\phi\sa^{\top}$. We denote the eigen-decomposition of $\Sigma_h$ as $\Sigma_h = U_h\Lambda_h U_h^{\top}$ with $U_h\in \mathbb{R}^{d\times d}$. Denote the eigen-vectors whose corresponding eigen values are no smaller than $\delta\in\mathbb{R}^+$ as $\{u_1,\dots, u_m\}$ with $0\leq m\leq d$. We denote $V_h = [u_1,\dots, u_m]\in\mathbb{R}^{d\times m}$. We abuse notation by using $V_h$ to denote the set $\{u_1,\dots, u_m\}$ and $\overline{V}_h$ the set of the rest eigen-vectors whose eigen-values are less than $\delta$.

Rmax gives us a \emph{explore-or-terminate} type result. The covariance matrix $\Sigma_h$ tells us which directions at time step $h$ have be well covered by $\rho_h$ and which directions are not. %The space that has not been covered by $\Sigma_h$ is denoted as the span of $\overline{V}_h$ ($\overline{V}_h$ contains eigen-vectors of $\Sigma_h$ whose eigen-values are small). 
Rmax algorithm calls FQI as the subroutines to try to find a policy that can escape to the span of $\overline{V}_h$. If FQI succeeds in terms of finding such policy, we add it to $\Pi_h$ the policy set and we make progress in a sense that we explore.  On the other hand, if FQI subroutines cannot find any policy that could escape to $\overline{V}_h$ for any $h\in [H]$, then it basically means that $\{\rho_{h}\}_{h=1}^H$ has already provide a good cover. At this stage, we call FQI with $\{\rho_h\}_{h=1}^H$ using the original reward of our MDP and terminate.  The returned policy from FQI is near optimal policy in terms of optimizing the original MDP. 



\begin{algorithm}[h]
	\begin{algorithmic}[1]	
		\Require The original MDP $M$ with reward $\boldr$; 
                \State Initialize H sets of policies: $\Pi_h = \{ \boldpi_h\}$ for all $h\in [H]$;
               	\For{ $e = 0, \dots, $}
			\State Define mixtures: $\rho_{h} := \frac{1}{|\Pi_h |} \sum_{\boldpi_h \in \Pi_h} d_h^{\boldpi_h}, \forall h\in [H]$.
			\For{$ h = 1, \dots H$} \Comment{check if we can escape}
				\For{ $v \in \overline{V}_h$ }
				\State Set  reward $\widetilde\boldr_h = \{r_1,\dots, r_h\}$ s.t. $r_i\sa =0$ for $i < h$ and $r_h\sa = \phi\sa\cdot v$;
				\State Set  reward $\widetilde\boldr'_h = \{r'_1,\dots, r'_h\}$ s.t. $r'_i\sa = 0$ for $i <h$ and $r'_h\sa =- \phi\sa\cdot v$;
				\State  $\{\widetilde{\boldpi}_{h}, V\} = \textrm{FQI}\left( \widetilde\boldr_h, h, \{\rho_i\}_{i=1}^{h-1} \right)$ and $\{\widetilde{\boldpi}'_h, V' \}=\textrm{FQI}\left(\widetilde\boldr'_h, h, \{\rho_i\}_{i=1}^{h-1} \right)$;
				\If{$\max\{ V, V'\} \geq \beta$}  \Comment{Escapes at direction $v$}
					\State $\Pi_h = \Pi_h  \oplus \{ \widetilde\boldpi_h, \widetilde\boldpi'_h \}$.
					\State \textbf{Break};
				\EndIf
				\EndFor
				\If{$\Pi_h$ is updated }
					\State \textbf{Break}
				\EndIf
			\EndFor
			\If{$h = H$}  \Comment{If cannot escape, call FQI \& terminate}
				\State \textbf{return} ${\boldpi} = \textrm{FQI}\left( \boldr, H, \{\rho_{h}\}_{h=1}^{H-1}\} \right)$;
			\EndIf
		\EndFor
         \end{algorithmic}
	\caption{Rmax}
\label{alg:rmax}
\end{algorithm}


\begin{algorithm}[!t]
	\begin{algorithmic}[1]	
		\Require rewards $\boldr$, horizon $h$, and restart distributions $\{\rho_1,\dots, \rho_{h-1}\}$; 
                \State Set $\widehat{Q}_{h}\sa = r_h\sa$ for all $\sa\in\Scal\times\Acal$
               	\For{ $\tau = {h-1}, \dots, 1$} \Comment{Dynamic Programming}
			\State Sample $N$ state-action-next state triples $\{s_i,a_i, s'_i\}_{i=1}^N$ where $(s_i,a_i)\sim \rho_{\tau}, s'_i\sim P_{s_i,a_i}$;
			%\State Compute $\widehat\theta_{\tau}$ that approximately minimizes $\EE_{\sa\sim \rho_{\tau}}\left( \theta\cdot\phi\sa - \Tcal\widehat{Q}_{\tau+1}\sa \right)^2$;
			\State $\widehat{\theta}_{\tau} := \arg\min_{\theta: \|\theta\|_2\leq W}\sum_{i=1}^N \left( \theta\cdot\phi(s_i,a_i) - r_{\tau}(s_i,a_i) - \max_{a'}\widehat{Q}_{\tau+1}(s_i', a') \right)^2$; \Comment{linear regression}
			%\State If $h = H$, \textbf{return} $\hat{\pi} = FQI\left( \{\rho_{e;h}\}_{h=1}^H, r, \text{horizon} = H\} \right)$;
			\State Denote $\widehat{Q}_{\tau}\sa = \widehat\theta_{\tau}\cdot\phi\sa$;
		\EndFor
		\State Set $\boldpi := \left\{ \pi_\tau(\cdot) := \arg\max_{a} \widehat{\theta}_\tau\cdot\phi(\cdot, a) \right\}_{\tau=1}^h$;
		\State Generate $M$ trajectories $\left\{\xi_i := \{s_\tau^{(i)},a_\tau^{(i)}\}_{\tau=1}^h \right\}_{i=1}^M$ using $\boldpi$ ; \Comment{Estimate $\EE_{\boldpi}[\sum_{\tau=1}^{h} r_\tau]$}
		\State Estimate expected total reward of $\boldpi$ as $\widehat{V} := \sum_{i=1}^M \sum_{\tau=1}^h r_\tau(s^{(i)}_\tau,a_\tau^{(i)})/M$;
	\State \textbf{Return} $\boldpi := \left\{ \pi_\tau(\cdot) := \arg\max_{a} \widehat{\theta}_\tau\cdot\phi(\cdot, a) \right\}_{\tau=1}^h$ and $\widehat{V}$;
         \end{algorithmic}
	\caption{Fitted Q-Iteration ($\boldr, h, \{\rho_1,\cdots, \rho_{h-1}\}$)}
\label{alg:fqi}
\end{algorithm}



Below we analyze the performance of Rmax. In~\pref{sec:fqi_analysis}, we start by showing that if $\{\rho_h\}_{h=1}^H$ provides a good cover over state-action space (\pref{assum:restart_distributions}), then FQI with $\{\rho_h\}$ returns a near-optimal policy (\pref{thm:psdp}). 

\subsection{FQI Analysis}
\label{sec:fqi_analysis}
Consider finite horizon $H$ and for each $h$ we have a restart distribution $\rho_{h}$. %of which the (uncentered) covariance is denoted as $\Sigma_h = U_h\Lambda_h U_h^{\top}$. 
We assume the following property of the restart distributions $\{\rho_h\}_{h=1}^H$. 
\begin{assum}
For any $h\in [H]$, denote the eigen-decomposition of $\Sigma_h$ as $\Sigma_h = U_h \Lambda_h U_h^{\top}$. Assume that $\Sigma_h \geq \delta V_hV_h^{\top}$ where $V_h = [u_1,\dots, u_m]$ contains eigen-vectors whose eigenvalues no smaller than $\delta$. For any $i > m$, we have that $\max_{\pi}\left\lvert  \EE_{\pi}\left[ \phi(s_h,a_h)^{\top} u_i  \right]\right\rvert \leq \beta_h \in\mathbb{R}^+$ for all $h\in [H]$. 
\label{assum:restart_distributions}
\end{assum}




\begin{theorem}  Under~\pref{assum:restart_distributions}, with $\{\rho_h\}_h$ as the restart distributions, FQI (\pref{alg:fqi}) returns a policy ${\boldpi}$,
\begin{align*}
V^{\star}- V^{\boldpi} \leq  H^2 \sqrt{\epsilon/\delta} + 2d  H W\sum_{h=1}^{H-1}\beta_{h},
\end{align*} where $\epsilon$ is the upper bound on the regression error, $\max_h \EE_{\sa\sim \rho_{h} }\left( \widehat\theta_h\cdot \phi\sa - \Tcal_h \widehat{Q}_{h+1}\sa \right)^2 \leq \epsilon$.
\label{thm:psdp}
\end{theorem}



\begin{proof}
Via Performance Difference Lemma, we have:
\begin{align}
 V^\star - V^{\boldpi} & = \sum_{h=1}^H \EE_{s\sim d_{h}^{\boldpi}}\left[ Q^\star_h(s, \pi^\star(s)) - Q^\star_h(s, \pi_h(s))\right] \nonumber \\
& \leq \sum_{h=1}^H \EE_{s\sim d_{h}^{\boldpi}}\left[ Q^\star_h(s,\pi^\star(s)) - \widehat{Q}_h(s, \pi^\star(s)) + \widehat{Q}_h(s, \pi_h(s)) - Q^\star_h(s, \pi_h(s)) \right] \nonumber\\
& =\underbrace{ \sum_{h=1}^H \EE_{s\sim d_{h}^{\boldpi},a=\pi^\star(s)}\left[Q^\star_h(s,a) - \widehat{Q}_h(s,a)\right]}_{\text{a}} + \underbrace{\sum_{h=1}^H \EE_{s\sim d_h^{\boldpi}, a= \pi_h(s)} \left[\widehat{Q}_h(s,a) - Q^\star_h\sa\right]}_{\text{b}}. \label{eq:pdl}
\end{align}
Below we focus on time step $h-1$, and consider bounding the two terms on the RHS of the above inequality individually by building a recursion formulaiton. 

%Below we bound $\EE_{s\in d_h^{\boldpi}}\left( Q^\star_h\sa - Q^\star_h(s,\pi_h(s)) \right)$ for each $h\in [H]$.

%Consider time step $h-1$. Denote $\widehat{Q}_h\sa = \widehat\theta_h\phi\sa$. 
Note that via Bellman completeness, there exists a $\theta_{h-1}$, s.t., 
\begin{align*}
\theta_{h-1}\cdot \phi\sa = r_h\sa + \EE_{s'\sim P_h(\cdot|s,a)} \max_{a'} \widehat{Q}_h(s',a') := \Tcal_h\widehat{Q}_h\sa.
\end{align*}  %Denote $\widehat{\pi}_h(s) = \arg\max_{a} \widehat{Q}_h(s,a)$.
Since $\widehat\theta_{h-1}$ is learnt by linear regression under $\rho_{h-1}$ with $\Tcal_h\widehat{Q}_h\sa$ as the regression target, we have:
\begin{align*}
\EE_{\sa\sim \rho_{h-1}} \left(\widehat\theta_{h-1}\cdot \phi\sa - \theta_{h-1}\cdot\phi\sa \right)^2\leq \epsilon \Rightarrow (\widehat\theta_{h-1}-\theta_{h-1})^{\top} V_{h-1}V_{h-1}^{\top}(\widehat\theta_{h-1} - \theta_{h-1}) \leq \frac{\epsilon}{\delta}.
\end{align*}
We first bound term $a$. Consider $Q^\star_{h-1}\sa - \widehat{Q}_{h-1}\sa$ for any $\sa$:
\begin{align*}
&  Q^\star_{h-1}\sa - \widehat{Q}_{h-1}\sa  =  \Tcal_h Q^\star_{h}\sa - \Tcal_h \widehat{Q}_{h}\sa  +  \Tcal_h \widehat{Q}_{h}\sa - \widehat{Q}_{h-1}\sa   \\
& = \EE_{s'\sim P_h(\cdot|s,a)} \left(Q^\star_{h}(s',\pi^\star(s')) -  \widehat{Q}_h(s',{\pi}_h(s'))\right)  + \Tcal_h \widehat{Q}_{h}\sa - \widehat{Q}_{h-1}\sa\\
& \leq \EE_{s'\sim P_h(\cdot|s,a), a' = \pi^\star(s')}\left( Q^\star_h(s', a') - \widehat{Q}_h(s', a') \right) + \Tcal_h \widehat{Q}_h\sa - \widehat{Q}_{h-1}\sa,
\end{align*} where in the last inequality we use the fact that $\widehat{Q}_h(s, \pi_h(s))\geq \widehat{Q}_h(s, \pi^\star(s))$ for any $s$.
Consider an arbitrary roll-in distribution $d_{h-1}$ that results from some policy. Add $\EE_{s\sim d_{h-1} }$ on both sides and take $a = \pi^\star(s)$,  we have:
\begin{align*}
&\EE_{s\sim d_{h-1},a=\pi^\star_s} \left(Q^\star_{h-1}\sa - \widehat{Q}_{h-1}\sa \right) \\
&\leq \EE_{s\sim d_{h-1},a=\pi^\star_s}\EE_{s'\sim P_h(s,a), a'=\pi^\star_{s'}} \left(Q^\star_h(s',a') - \widehat{Q}_h(s',a') \right) + \EE_{s\sim d_{h-1}, a=\pi^\star_s}\left( \Tcal_h\widehat{Q}_h\sa - \widehat{Q}_{h-1}\sa \right) \\
& := \EE_{s\sim d_{h}, a=\pi^\star_s}\left( Q^\star_h(s,a) - \widehat{Q}_h\sa \right) + \underbrace{\EE_{s\sim d_{h-1}, a=\pi^\star_s}\left( \Tcal_h\widehat{Q}_h\sa - \widehat{Q}_{h-1}\sa \right)}_{\text{regression error}},
\end{align*} where in the last inequality we denote $d_h(s') := \sum_{s} d_{h-1}(s)P_h(s'|s,\pi^\star_s)$. Now we argue the the term \emph{regression error} cannot be too big:
\begin{align*}
&\EE_{s\sim d_{h-1}, a= \pi^\star_s} \left( \Tcal_h \widehat{Q}_h\sa - \widehat{Q}_{h-1}\sa \right)= \EE_{s\sim d_{h-1}, a = \pi^\star_s} \left( \phi\sa\cdot ( \theta_{h-1} - \widehat\theta_{h-1} ) \right) \\
&=  \EE_{s\sim d_{h-1}, a= \pi^\star_s}  \left(  \proj_{V_{h-1}} \phi\sa \cdot ( \theta_{h-1} - \widehat\theta_{h-1} )  \right) +  \EE_{s\sim d_{h-1}, a =  \pi^\star_s}  \left(  \proj_{\overline{V}_{h-1}} \phi\sa \cdot ( \theta_{h-1} - \widehat\theta_{h-1} )  \right) \\
& \leq \sqrt{\EE_{s\sim d_{h-1}, a =\pi^\star_s}\left( \proj_{V_{h-1}}\phi\sa\cdot (\theta_{h-1}-\widehat{\theta}_{h-1}) \right)^2   }  + \sum_{v\in \overline{V}_{h-1}}\left( v\cdot (\theta_{h-1}-\widehat{\theta}_{h-1})\right) \EE_{s\sim d_{h-1}, a= \pi^\star_s} \left[\phi\sa\cdot v \right]\\
& \leq \sqrt{\frac{\epsilon}{\delta}} + \sum_{v\in\overline{V}_{h-1}} 2W \left\lvert \EE_{s\sim d_{h-1},a= \pi^\star_s} \phi\sa\cdot v \right\rvert \leq \sqrt{\frac{\epsilon}{\delta}} + 2dW \beta_{h-1},
\end{align*} where in the last inequality, we use the assumption that $\|\theta_{h-1}\|_2\leq W$, $\|\widehat{\theta}_{h-1}\|_2\leq W$ and $\max_{\boldpi}\EE_{\boldpi}\left[ \phi(s_{h-1},a_{h-1})\cdot v \right] \leq \beta_{h-1}$ for any $v\in \overline{V}_{h-1}$. This give us the following recursion formulation:
\begin{align*}
\EE_{s\sim d_{h-1},a=\pi^\star_s} \left(Q^\star_{h-1}\sa - \widehat{Q}_{h-1}\sa \right) \leq \EE_{s\sim d_h,a=\pi^\star_s} \left( Q^\star_h\sa - \widehat{Q}_h\sa \right) + \sqrt{\epsilon/\delta} + 2dW \beta_{h-1}.
\end{align*} Now we can keep expanding the RHS of the above inequality all the way to $H$, and we will get:
\begin{align*}
\EE_{s\sim d_{h-1},a=\pi^\star_s} \left(Q^\star_{h-1}\sa - \widehat{Q}_{h-1}\sa \right) \leq (H-h)\sqrt{\epsilon/\delta} + 2dW \sum_{\tau = h-1}^{H-1} \beta_\tau.
\end{align*}
Since the above inequality holds for any roll-in $d_{h-1}$, it holds for $d_{h-1}^{\boldpi}$, which concludes the derivation of upper bounding term $a$ in~\pref{eq:pdl}. 

We can perform similar analysis on bounding term $b$ in~\pref{eq:pdl}, and we can get:
\begin{align*}
\EE_{s\sim d_{h-1}, a = \pi_h(s)} \left[ \widehat{Q}_h\sa - Q^\star_h\sa \right] \leq (H-h) \sqrt{\epsilon/\delta} + 2Wd \sum_{\tau = h-1}^{H-1} \beta_{\tau},
\end{align*} which also holds for any roll-in distribution $d_{h-11}$ including $d_{h-1}^{\boldpi}$. 

Now we can go back to~\pref{eq:pdl} to conclude:
\begin{align*}
V^\star - V^{\boldpi} \leq \sum_{h} \left((H-h) \sqrt{\epsilon/\delta} +  2Wd \sum_{\tau = h}^{H-1}\beta_\tau \right) \leq H^2\sqrt{\epsilon/\delta} + 2dWH \sum_{h=1}^{H-1}\beta_h. 
\end{align*}

\end{proof}

The above theorem shows for restart distributions such that there is no policy that could reach the subspace where $\rho_{h}$ does not cover (i.e., $\beta_h$ is small) and linear regression in FQI succeeds (i.e., $\epsilon$ is small), then FQI will find a near-optimal policy.




\wen{stuff below here has not be corrected or refined....}
\section{Algorithm for Checking Termination Conditions}
We have the following information available. We have a sequence of restart distribution $\{\rho_h\}_{h=1}^H$ each has uncentered covariance denoted as $\Sigma_h = U_h^{\top} \Lambda_h U_h^{\top} \geq \delta V_h V_h^{\top}$ where $V_h$ is the eigenvectors in $U_h$ whose eigen-values no smaller than $\delta$.  We denote $\overline{V}_h$ as the rest of the eigen-vectors in $U_h$.

We terminate Rmax algorithm if the following condition holds: 
\begin{align*}
\forall h\in [H], \forall u \in \overline{V}_h, \max_{\pi} \left\lvert\EE_{\pi}\left[ \phi(s_h,a_h)\cdot u  \right] \right\lvert \leq \beta.
\end{align*}
%\wen{this condition works, if $\phi\sa \cdot u$ is non-negative and less than 1, which is true if features are positive and we use standard basis..}

Below, we focus on how to compute $\max_{\pi} \EE_{\pi}\left[ \phi(s_h,a_h)\cdot u \right]$ and $\max_{\pi} \EE_{\pi}\left[ -\phi(s_h,a_h)\cdot u \right]$. 
\begin{theorem} Assume that for any $\tau < h$ and $v\in \overline{V}_\tau$, we have $\max_{\pi} \EE_{\pi}\left[ (\phi(s_{\tau},a_{\tau})\cdot v)^2\right] \leq \beta$.  Run FQI with $\{\rho_1,\dots, \rho_{h-1}\}$ as the restart distribution and $r_h\sa := \phi\sa\cdot v$ and $r_{\tau}\sa = 0$ as the rewards. FQI returns a policy $\widehat\pi$ such that:
\begin{align*}
\EE_{\widehat{\pi}}\left[ \phi(s_h,a_h)\cdot v \right] \geq \max_{\pi}\EE\left[ \phi(s_h,a_h)\cdot v\right] - h^2 \sqrt{2\epsilon/\delta + 2dW\beta}.
\end{align*} where $\epsilon$ is the regression error.
\end{theorem}
\begin{proof} 
Denote $\pi^\star := \arg\max_{\pi} \EE_{\pi} [\phi(s_h,a_h)\cdot v]$.

Note that $Q^\star_h\sa = \phi\sa\cdot v$ is known and is linear wrt $\phi\sa$. FQI starts with $Q^\star_h$ directly, i.e., $\widehat{Q}_h\sa = \phi\sa\cdot v = Q^\star_h\sa$.

Now let us consider time step $\tau$. Assume that $\widehat{Q}_{\tau+1}\sa = \widehat\theta_{\tau+1}\cdot \phi\sa$ (note this linearity holds when $\tau+1 = h$). Via Completeness, we have that:
\begin{align*}
\Tcal \widehat{Q}_{\tau+1}\sa = \theta_{\tau}\cdot \phi\sa.
\end{align*} As FQI learns $\widehat{\theta}_{\tau}$ via linear regression under $\rho_{\tau}$ with $\Tcal \widehat{Q}_{\tau+1}\sa$ as the regression target, we have:
\begin{align*}
\EE_{\sa\sim \rho_{\tau}} \left( (\widehat\theta_\tau - \theta_\tau)\cdot\phi\sa \right)^2 \leq \epsilon \Rightarrow \left(\widehat\theta_\tau - \theta_\tau\right)V_{\tau}V_{\tau}^{\top} \left(\widehat\theta_\tau - \theta_\tau\right) \leq \frac{\epsilon}{\delta}.
\end{align*}
Consider $\phi(s_\tau,a_\tau)\cdot (\widehat\theta_\tau - \theta_\tau)$:
\begin{align*}
&\left\lvert \phi(s_\tau,a_\tau)\cdot (\widehat\theta_\tau - \theta_\tau) \right\rvert^2 \leq 2 \left\lvert \proj_{V_\tau}\phi(s_\tau,a_\tau)\cdot (\widehat\theta_\tau - \theta_\tau) \right\rvert^2 + 2\left\lvert\proj_{\overline{V}_\tau}\phi(s_\tau,a_\tau)\cdot (\widehat\theta_\tau - \theta_\tau)\right\rvert^2 \\
& \leq \frac{2 \epsilon}{\delta} +  2W \sum_{v\in \overline{V}_{\tau}} (\phi(s_\tau,a_\tau)\cdot v)^2
\end{align*} Hence, for any roll-in policy $\pi$, we have:
\begin{align*}
\EE_{\pi}\left( \phi(s_\tau,a_\tau)\cdot (\widehat\theta_\tau - \theta_\tau) \right)^2 \leq \frac{2\epsilon}{\delta} + 2d W \beta, 
\end{align*} where we use the assumption that $\max_{\pi} \EE_{\pi}\left( \phi(s_\tau,a_\tau)\cdot v \right)^2 \leq \beta$ for any $v\in \overline{V}_\tau$ and any $\tau < h$.

%Now consider the following quantity:
Similar to the FQI analysis above, we can have the following recursion:
\begin{align*}
&\EE_{s\sim \nu_{\tau}, a\sim \pi} \left\lvert  Q^\star_\tau\sa - \widehat{Q}_\tau\sa \right\rvert \\
& \leq \EE_{s\sim \nu_\tau, a\sim \pi}\EE_{s'\sim p\sa} \left\lvert Q^\star_{\tau+1}(s', \pi^\star(s')) - \widehat{Q}_{\tau+1}(s', \widehat{\pi}_h(s')) \right\rvert + \sqrt{2\epsilon/\delta + 2dW\beta} \\
& \leq \EE_{s\sim \nu_{\tau+1}}\max_{a} \left\lvert Q^\star_{\tau+1}\sa - \widehat{Q}_{\tau+1}\sa \right\rvert + \sqrt{2\epsilon/\delta + 2dW\beta} \\
& \leq (h-\tau) \sqrt{2\epsilon/\delta + 2dW\beta}.
\end{align*}
Using performance difference lemma allows us the conclude the proof. 
\end{proof}










==> docs/sketch.tex <==
\section{Setting}

We denote the ground truth MDP as $\Mcal = \{\Scal,\Acal, P, \gamma, c, s_0\}$.   We assume that we have an expert policy $\pi^e: \Scal\mapsto \Delta(\Acal)$. Here cost function $c$ is only state dependent, i.e., $c:\Scal\mapsto [0,1]$. We consider the setting where $\Acal$ is discrete. We denote $A = |\Acal|$. Here $s_0$ is an initial fixed state, and learner can reset to and only to this initial state $s_0$.  

We can ask expert to provide a state-only demonstration trajectory $\tau = \{s_0, s_1 \dots s_t,\dots \}$, where $s_{t+1} \sim P(\cdot | s_t, a_t)$ and $a_t \sim \pi^\star(\cdot | s_t)$.  Note that the expert demonstration always starts from $s_0$. Unlikely interactive imitation learning (e.g., DAgger and AggreVaTe), we cannot ask expert to provide demonstration starting from any state. 

While the true $r$ is unknown to the learner, we assume that we have a function class $\Fcal\subset \Scal\mapsto [0,1]$.  We assume realizability, i.e., $c\in \Fcal$.

For transition $P$ and function $f: \Scal\mapsto [0,1]$,  and a policy $\pi:\Scal\mapsto\Delta(\Acal)$, we will define $V^{\pi}_{P,f}$ as the value function of policy $\pi$ under transition $P$ and ``reward" function $f$.







\section{Algorithm Description}


\subsection{Absorbing MDP construction}
Assume that we are given a known set over state space $\Kcal \subset \Scal$. We define the following absorbing MDP:
\begin{align*}
P^\dagger(\cdot | s,a) = \begin{cases}
P(\cdot | s,a) & s \in\Kcal; \\
\delta_{s} & s \not\in\Kcal.
\end{cases} 
\end{align*} Namely, we will self-loop at $s$ when $s\not\in\Kcal$.
%Note here we denote $s^\dagger \not\in\Kcal$. 

We also need to define the corresponding absorbing MDP using our learned model $\widehat{P}$: \begin{align*}
\widehat{P}^\dagger(\cdot | s,a) = \begin{cases}
\widehat{P}(\cdot | s,a) & s \in\Kcal; \\
\delta_{s} & s \not\in\Kcal.
\end{cases} 
\end{align*}
Let us assume the following state-action wise model error bound for states in  $\Kcal$:
\begin{align*}
\forall s\in \Kcal: \left\| \widehat{P}(\cdot | s,a) - P(\cdot | s,a)     \right\|_{tv} \leq \epsilon_{stat}, \forall a\in\Acal.
\end{align*}

Using simulation lemma (\pref{lem:simulation}), for any $f$ with $f(s,a)\in [0,1]$ for all $s,a$, and $\pi$, we will have:
\begin{align*}
\left\lvert \mathbb{E}_{s\sim d^{\pi}_{\widehat{P}^\dagger} }f(s) - \mathbb{E}_{s'\sim d^{\pi}_{P^\dagger}}f(s)    \right\rvert \leq \frac{1}{1-\gamma} \mathbb{E}_{s,a\sim d^{\pi}_{P^\dagger}} \one\{s\in\Kcal\} \left\| \widehat{P}(\cdot | s,a) - P(\cdot|s,a)  \right\|_{tv} \leq \frac{\epsilon_{stat}}{1-\gamma}.
\end{align*}

Given some cost function $c$, we also define the corresponding truncated cost $c^\dagger$ using $\Kcal$:
\begin{align*}
c^\dagger(s) = \begin{cases}
c(s), & s\in\Kcal, \\
0, & s\not\in\Kcal.
\end{cases}
\end{align*}

Given the definition of $c^\dagger$ above, we define $\Fcal^\dagger$ as follows:
\begin{align*}
\Fcal^{\dagger} = \{f^\dagger: f \in \Fcal \}.
\end{align*}




\subsection{Simulate  $\pi^e$ on $P^\dagger$}
\begin{algorithm}[t]
\begin{algorithmic}[1]
%\setcounter{algorithm}{-1}
\Function{Sample}{}
\State  \hspace*{-0.1cm}\textbf{Input}:  $\pi, \M, \Kcal$
%\State Sample $s_0,a_0 \sim \rho_0\times\pi$
\State Reset to $s_0$
\State Sample a time step $h \propto \gamma^h$ from $[0, \infty]$
\State Ask $\pi^e$ for a length $h+1$ demonstration in $\Mcal$: $\{s_0, a_0,\dots, s_h,a_h \}$ \Comment{Actions are not observed by learner}
\State \textbf{Return} $s_h$ if $\forall \tau\in [0,h-1], s_\tau\in\Kcal$
\State Otherwise, set $t = \min\{t\in [h]: s_{t} \not\in\Kcal\}$, and return $s_t$. 
%\State \textbf{Return} $s_h$ if $\forall \tau\in [0,h-1], s_\tau\in\Kcal$; otherwise \textbf{return} $s^\dagger$
%\For{$t = 0 \dots$}	
%\EndFor
%\State At any time step $t$, stop with probability $1-\gamma$ or if $s_t\not\in\Kt$, else, $s_{t+1},a_{t+1}\sim P(\cdot|s_t,a_t)\times\pi$.
%\State  \hspace*{-0.1cm}\textbf{Return}: $s_t$, $\text{True}$ if $s_t\not\in\Kt$ else $\text{False}$.
\caption{Simulated $d^{\pi^e}_{P^\dagger}$ state-sampler}
\EndFunction
\label{alg:sampling_absorbing}
\end{algorithmic}
\end{algorithm}
Given the absorbing MDP $P^\dagger$, and the expert policy $\pi^e$, we can simulate a state sampling oracle from $d^{\pi^e}_{P^\dagger}$ in \pref{alg:sampling_absorbing}, by asking $\pi^e$ to provide a demonstration starting from $s_0$ at the original transition $P$.  While the expert is not aware of the absorbing structure, from the perspective of the sampler (\pref{alg:sampling_absorbing}), once it observes that the expert trajectory enters $\Kcal$ at some step $t$, it can just return $s_t$ regardless of what future states the expert generates, since from the absorbing MDP's perspective, we will self-loop at $s_t$ forever since $s_t\not\in\Kcal$.  

Calling \pref{alg:sampling_absorbing} once with $(P, \Kcal)$ as input, we get a sample $s$ from $d^{\pi^e}_{P^\dagger}$ with $P^\dagger$ defined with respect to $\Kcal$.


%Note that the expert $\pi^e$ is not aware of $P^\dagger$ and we can only execute $\pi^e$ from $s_0$ at the ground truth MDP transition $P$, and we do not get to observe expert's action. \wen{We can verify that \pref{alg:sampling_absorbing} is equivalent to $s\sim d^{\pi^e}_{P^\dagger}$}. 


\subsection{Algorithm}

In \pref{alg:main_alg},  we first define known state-action set according to Line 7. We abuse the notation slightly by defining known set for states $\Kcal = \{s: \forall a, s,a\in \Kcal\}$, i.e., a state is called known if and only if for all action $a$, $s,a$ is known. 

In Line 6, we do modeling fit under all historical policies' distributions. We simply perform MLE on the model class. For KNRs, the model class consists of Gaussian models with mean being linear functions with respect to $\phi$, i.e., $\Pcal = \left\{  P(\cdot | s,a) := \mathcal{N}\left( W\phi(s,a), \sigma^2 I \right), \forall s,a : \|W\|_2 \leq C \right\}$. In this case, the MLE objective simply reduces to least square regression:
\begin{align*}
\argmin_{W: \|W\|_2\leq C} \sum_{i} \| W\phi(s_i,a_i) - s_i' \|^2_2.
\end{align*}

We perform model-based planning in Line 9, where the discriminators $\Fcal^\dagger_t$ is defined using $\Kcal_t$, and the absorbing transition $\widehat{P}_t^\dagger$ is defined using $\Kcal_t$ and $\widehat{P}_t$.

\begin{algorithm}[t]
\begin{algorithmic}[1]
\caption{Main Algorithm}
\State \textbf{Input}: Model class $\Pcal$, policy class $\Pi$; parameter $\beta, K, T, M, N$
\State Initialize policy $\pi_1\in\Pi$ to be a uniform random policy and a policy cover $\boldpi_1 = \{\pi_1\}$
\For{$t = 1 \to T$}
	\State Draw $K$ samples $\{s_i,a_i\} \sim d^{\pi_t}$
	\State Set $\widehat{\Sigma}_{\pi_n} = \sum_{i=1}^K \phi(s_i,a_i)\phi(s_i,a_i)^{\top} /K$
	\State Set covariance matrix $\widehat{\Sigma}_t = \sum_{i=1}^t \widehat\Sigma_i + \lambda I$
	\State Set $\widehat{P}_t$ as the approximate MLE of the following log-likelihood objective:
	\begin{align*} \min_{P\in\Pcal} \sum_{i=1}^M \ln P(s_i'|s_i,a_i), \end{align*} where $\{s_i,a_i,s_i'\}$ are sampled as $(s_i,a_i)\sim d^{\boldpi_t}$, $s_i'\sim P(\cdot | s_i,a_i)$; \Comment{Model-fitting under all historical policies} \label{line:model_fitting}
	\State Define $\Kcal_t = \left\{s,a: \phi(s,a)^{\top} \widehat{\Sigma}_t^{-1}\phi(s,a) \leq \beta_t \right\}$ \label{line:known_state_action}
	\State Call $d^{\pi^e}_{P^\dagger}$-sampler (\pref{alg:sampling_absorbing} with $\Kcal_t$) N times to get $\{s^e_i\}_{i=1}^N \sim d^{\pi^e}_{P^\dagger}$ i.i.d samples
	\State Planning $\widehat{\pi}_{t+1} = \argmin_{\pi\in\Pi} \max_{f\in \Fcal_t^{\dagger}} \left[ \mathbb{E}_{s\sim d^{\pi}_{\widehat{P}_t^\dagger}} f(s) - \sum_{i=1}^N f(s^e_i) / N   \right] $ \Comment{Model-based Planning} 
	\State Define $\pi_{t+1}(\cdot | s) = \begin{cases} \widehat{\pi}_{t+1}(\cdot | s) & s\in\Kcal_t\\
	\text{Uniform}(\Acal) & \text{ else}.
	\end{cases}$, and append to policy cover $\boldpi_{t+1} = \boldpi_t + \{\pi_{t+1}\}$
\EndFor
%\EndFunction
\label{alg:main_alg}
\end{algorithmic}
\end{algorithm}



\section{Analysis}

%{I think we should do model-based planning here, i.e., we can do: $\min_{\pi\in\Pi}\| d^{\pi}_{\widehat{P}^\dagger} - d^{\pi^e}_{P^\dagger}  \|_{tv}$. Note that here we have $\widehat{P}$ for our policy $\pi$ and $P^\dagger$ for $\pi^e$. But $\widehat{P}^\dagger$ and $P^\dagger$ are close for any state-action pair. Optimize TV directly is not feasible, so we can minimize IPM here with the modified discriminator class $\Fcal^\dagger$:
%\begin{align}
%\label{eq:IPM}
%\min_{\pi\in \Pi}\max_{f\in\Fcal^\dagger} \left[ \EE_{s\sim d^{\pi}_{\widehat{P}^\dagger}}f(s) - \widehat{\EE}_{s\sim d^{\pi^e}_{P^\dagger}}[f(s)]  \right],
%\end{align} where we denote $\widehat{\EE}$ as the empirical approximation of $\EE$, and $\Fcal^\dagger = \{f \in \Fcal: f(s,a) = 0, \forall s \not\in\Kcal\}$. Note that $\Fcal^\dagger$ contains the truncated cost function:
%\begin{align*}
%c^\dagger(s) = \begin{cases}
%c(s), & s\in\Kcal, \\
%0, & s\not\in\Kcal.
%\end{cases}
%\end{align*}
% We can do following the leader on $\pi$ which uses a pure planning oracle, and best response on $f$.
%}
%\iffalse
%\begin{algorithm}[H]
%\begin{algorithmic}%[1]
%\setcounter{algorithm}{-1}
%\Function{Policy Update}{}
%\State  \hspace*{-0.1cm}\textbf{Input}:  $\D\equiv\{s_i,a_i,s'_i,\mu(a_i|s_i)\}_{i=1}^N, \D_e\equiv\{s^e_i\}_{i=1}^{N'},\pi_0$.
%\State Define $u(\pi,f):=\mathbb{E}_{(s,a,s')\sim\D}[\frac{\pi(a|s)}{\mu(a|s)}\cdot f(s')]-\mathbb{E}_{s''\sim\D_e}[f(s'')]$, where, $K=|\mathcal{A}|$.
%\For{$t=0,1,\cdots$}
%\State $f^t\leftarrow \arg\max_{f\in\mathcal{F}}u(\pi_n,f)$.
%\State $u^n\leftarrow u(\pi_n,f^n)$.
%\State $\pi_{n+1}\leftarrow \sum_{t=1}^n u(\pi,f^t) + \phi(\pi)$.
%\EndFor
%\State  \hspace*{-0.1cm}\textbf{Return}: $\pi_t$, where, $t=\arg\min_j u^j$.
%\caption{Policy Updater}
%\EndFunction
%\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}[H]
%\begin{algorithmic}%[1]
%\setcounter{algorithm}{-1}
%\Function{Sample}{}
%\State  \hspace*{-0.1cm}\textbf{Input}:  $\mathcal{F},\epsilon$
%\State $\D,\D_e, T, \K_0,\pi_0\leftarrow \{\},\{\}, \tilde{\mathcal{O}}(1/\epsilon),\{\text{UNK}\},\text{Unif}(|\mathcal{A}|)$.
%\For{$t=0,1,\cdots$}
%\For{$j=0,1,\cdots,T$}
%\State $s_j,p_j\leftarrow \text{SAMPLE}(\pi_e,\M,\K_t)$
%\State $\D_e\leftarrow \D_e\cup\{s_j\}$
%\If{$p_j==\text{True}$}
%\State Break
%\EndIf
%\EndFor
%\If{$\{p_j\}==\text{False}\ \forall j$}
%\State Break
%\EndIf
%\While{$s_j\not\in\K_t$}
%\State Get $\mathcal{S}'=(s,a)$ pairs by making $\pi$ interact with $\M$.
%\State $\D\leftarrow\D\cup\mathcal{S}'$.
%\State Update $\K_t$.
%\EndWhile
%\State $\pi_{t+1}\leftarrow\text{POLICY Update}(\D,\D_e)$
%\EndFor
%\State  \hspace*{-0.1cm}\textbf{Return}: $\pi_{t+1}$.
%\caption{Overall Algorithm}
%\EndFunction
%\end{algorithmic}
%\end{algorithm}
%\fi

\subsection{When can we terminate?}

We terminate when our learned policy $\pi$ does not escape, i.e., $\sum_{s\not\in\Kcal} d_P^{\pi}(s) \leq \epsilon$.

\begin{lemma} Consider any policy $\pi$.  Assume that $\sum_{s\not\in\Kcal} d_P^{\pi}(s) \leq \epsilon$.  Then, for any $f: \Scal\mapsto [0,1]$, we have:
\begin{align*}
\left\lvert \mathbb{E}_{s\sim d_P^{\pi}} f(s) - \mathbb{E}_{s\sim d^{\pi}_{P^\dagger}}f(s)\right\rvert \leq 2\epsilon.
\end{align*}\label{lem:link_known_unknown}
\end{lemma}
\begin{proof}
From Simulation Lemma (\pref{lem:simulation}) we have:
\begin{align*}
\left\lvert \mathbb{E}_{s\sim d_P^{\pi}} \left[ f(s)\right] - \mathbb{E}_{s\sim d^{\pi}_{P^\dagger}}\left[ f(s)\right]\right\rvert  &  \leq  \mathbb{E}_{s,a\sim d^{\pi}_{P}}\one\{s\in\Kcal\} \| P^\dagger_{s,a} - P_{s,a}   \|_1 +  \mathbb{E}_{s,a\sim d^{\pi}_{P}}\one\{s\not\in\Kcal\} \| P^\dagger_{s,a} - P_{s,a}   \|_1 \\
& \leq  2 \mathbb{E}_{s,a\sim d^{\pi}_P} \one\{s\not\in\Kcal\} = 2 \sum_{s\not\in\Kcal} d^{\pi}_P(s) \leq 2\epsilon. 
\end{align*}
\end{proof}


\begin{lemma}[Optimistic Estimate]
\label{lem:optimism}
Consider any policy $\pi$. Under the model $\left( P^\dagger, c^\dagger \right)$ and the model $(P, c)$, we have:
\begin{align*}
V^{\pi} \geq V^{\pi}_{P^\dagger,c^\dagger}.
\end{align*}
\end{lemma}
\begin{proof}
This is because in the absorbing MDP $P^\dagger$ and $c^\dagger$, once we hit an unknown state $s$, we self-loop and pay cost zero afterwards. 
\end{proof}

Now consider the following condition where we assume that we have successfully minimized IPM (the min-max objective Eq.~\ref{eq:IPM}), i.e., let us assume that from Eq.~\ref{eq:IPM}, we get a policy $\pi$ such that:
\begin{align}
\max_{f\in \Fcal^\dagger} \left[ \EE_{s\sim d^{\pi}_{P^\dagger}}f(s) - \EE_{s\sim d^{\pi^e}_{P^\dagger}}f(s) \right] \leq  \varepsilon_{\text{ipm}}.
\label{eq:ipm_condition}
\end{align} Note that $ \varepsilon_{\text{ipm}}$ contains model error from $\widehat{P}^\dagger$ and $P^\dagger$ and also the finite sample error from $\widehat{\EE}_{s\sim d^{\pi^e}_{P^\dagger}}$.

The following lemma indicates that if we terminate, i.e., $\sum_{s\not\in\Kcal} d_P^{\pi}(s) \leq \epsilon$, we have learned a good policy. 
\begin{lemma}[Quality of policy at Termination] Assume for $\pi$, we have Inequality.~\ref{eq:ipm_condition} holds, and also $\sum_{s\not\in\Kcal} d_P^{\pi}(s) \leq \epsilon$. We must have:
\begin{align*}
V^{\pi} \leq V^{\pi^e} + 3\epsilon + \varepsilon_{\text{ipm}}.
\end{align*}
\end{lemma}
\begin{proof}
First, from \pref{lem:link_known_unknown}, we know that with $f$ being set to the  cost $c^\dagger$, we have:
\begin{align*}
\left\lvert V^{\pi}_{P;c^\dagger} - V^{\pi}_{P^\dagger; c^\dagger} \right\rvert \leq 2 \epsilon. 
\end{align*} 
Also for $V^{\pi}$ and $V^{\pi}_{P;c^\dagger}$, we have:
\begin{align*}
\left\lvert V^{\pi} - V^{\pi}_{P; c^\dagger} \right\rvert \leq \sum_{s\not\in\Kcal} d^{\pi}_P(s) c(s) \leq \epsilon.
\end{align*}

Now use \pref{lem:optimism}, we get:
\begin{align*}
V^{\pi^e} \geq V^{\pi^e}_{P^\dagger;c^\dagger}.
\end{align*} Recall that $c^\dagger \in \Fcal^\dagger$, by the IPM assumption, we must have:
\begin{align*}
| V^{\pi}_{P^\dagger;c^\dagger} - V^{\pi^e}_{P^\dagger; c^\dagger} | \leq \varepsilon_{\text{ipm}}.
\end{align*} Thus, combine these inequalities together, we get:
\begin{align*}
V^{\pi^e} \geq V^{\pi^e}_{P^\dagger;c^\dagger} \geq V^{\pi}_{P^\dagger;c^\dagger} - \varepsilon_{\text{ipm}} \geq V_{P; c^\dagger}^{\pi} - 2\epsilon - \varepsilon_{\text{ipm}} \geq V^{\pi} - 3\epsilon - \varepsilon_{\text{ipm}} 
\end{align*}Rearrange, we conclude the proof. 
\end{proof}


\subsection{Why we make progress when the algorithm is not terminated}




For any policy $\pi$, we denote $\pi_{\Kcal}$ as the following policy:
\begin{align*}
\pi_{\Kcal}(\cdot | s) = \begin{cases}
\pi(\cdot | s), & s\in\Kcal, \\
\text{Unifm}_{\Acal}, & \text{else}.
\end{cases}
\end{align*}

Recall that we denote $s\in \Kcal$ if and only if $s,a\in \Kcal$ for all $a$.



So in this case, we have:
\begin{align*}
 \sum_{s,a \not\in\Kcal} d^{\pi_{\Kcal}}_{P^\dagger}(s,a) & = \sum_{s\not\in\Kcal} d^{\pi_{\Kcal}}_{P^\dagger}(s)  \sum_{a: (s,a)\not\in\Kcal} (1/A) = \sum_{s\not\in\Kcal} d^{\pi}_{P^\dagger}(s)  \sum_{a: (s,a)\not\in\Kcal} (1/A)  \geq \frac{1}{A} \sum_{s\not\in\Kcal} d^{\pi}_{P^\dagger}(s),
\end{align*} where the second equality uses the fact that for $s\not\in\Kcal$, we simply have $d^{\pi_{\Kcal}}_{P^\dagger}(s) = d^{\pi}_{P^\dagger}(s)$, and the last inequality uses the fact that for $s\not\in\Kcal$, by definition, there exists at least one action such that $(s,a)\not\in\Kcal$.

With Rmax-Lemma (\pref{lem:rmax}), together we get: 
\begin{align*}
\frac{1}{A} \sum_{s\not\in\Kcal}  d^{\pi_{\Kcal}}_{P}(s) \leq \frac{1}{A} \sum_{s\not\in\Kcal}  d^{\pi_{\Kcal}}_{P^\dagger}(s) \leq  \sum_{s,a\not\in\Kcal} d^{\pi_{\Kcal}}_{P^\dagger}(s,a) \leq \frac{1}{1-\gamma} \sum_{s,a\not\in\Kcal}d^{\pi_{\Kcal}}_{P}(s,a).
\end{align*}

If the algorithm does not terminate, then we must have $\sum_{s\not\in\Kcal} d^{\pi_{\Kcal}}_P(s) \geq \epsilon$, which implies that:
\begin{align*}
\sum_{s,a\not\in\Kcal}  d^{\pi_{\Kcal}}_{P}(s,a)\geq \frac{\epsilon(1-\gamma)}{A}.
\end{align*}

Non-trivial escaping probability implies that following non-trivial progress on the potential function:
\begin{align*}
\EE_{s,a\sim d^{\pi_{\Kcal}}} \left[ \phi(s,a)^{\top} \Sigma_n^{-1} \phi(s,a)\right] &\geq \EE_{s,a\sim d^{\pi_{\Kcal}}} \one\{s,a\not\in\Kcal\} \left[ \phi(s,a)^{\top} \Sigma_n^{-1} \phi(s,a)\right] \\
&  \geq \EE_{s,a\sim d^{\pi_{\Kcal}}} \one\{s,a\not\in\Kcal\}  \beta = \beta \sum_{s,a\not\in\Kcal} d^{\pi_{\Kcal}}(s,a) = \frac{\beta \epsilon (1-\gamma)}{ A}.
\end{align*}




%\section{The feature selection setting with low rank MDP}

\section{Analysis using Reward Bonus}

\begin{algorithm}[t]
\begin{algorithmic}[1]
\caption{Main Algorithm w/ Reward Bonus}
\State \textbf{Input}: Model class $\Pcal$, policy class $\Pi$; Expert dataset $\{{s}^e_i\}_{i=1}^N$
\State Initialize policy $\pi_1\in\Pi$
\State Initialize replay buffer $\Dcal = \emptyset$
\For{$t = 1 \to T$}
	\State Execute $\pi_t$ to generate a trajectory $\tau = \{s_0, a_0,\dots, s_{H-1}, a_{H-1}, s_H\}$
	\State Augment dataset $\Dcal = \Dcal  + \{ s_t, a_t, s_{t+1}   \}_{t=0}^{H-1}$
	%\State Set $\widehat{P}_t$ as the approximate MLE of the following log-likelihood objective:
	\State Fit model $\widehat{P}_t$ from $\Dcal$ and set bonus $b_t$
	%\begin{align*} \min_{P\in\Pcal} \sum_{i=1}^M \ln P(s_i'|s_i,a_i), \end{align*} where $\{s_i,a_i,s_i'\}$ are sampled as $(s_i,a_i)\sim d^{\boldpi_t}$, $s_i'\sim P(\cdot | s_i,a_i)$; \Comment{Model-fitting under all historical policies} \label{line:model_fitting}
	%\State Define $\Kcal_t = \left\{s,a: \phi(s,a)^{\top} \widehat{\Sigma}_t^{-1}\phi(s,a) \leq \beta_t \right\}$ \label{line:known_state_action}
	\State Planning $\pi_{t+1} = \argmin_{\pi\in\Pi} \max_{f\in \widetilde{F}_t} \left[ \mathbb{E}_{s\sim d^{\pi}_{\widehat{P}_t}} f(s) - \sum_{i=1}^N f(s^e_i) / N  \right] $
	%\State Call $d^{\pi^e}_{P^\dagger}$-sampler (\pref{alg:sampling_absorbing} with $\Kcal_t$) N times to get $\{s^e_i\}_{i=1}^N \sim d^{\pi^e}_{P^\dagger}$ i.i.d samples
	%\State Planning $\widehat{\pi}_{t+1} = \argmin_{\pi\in\Pi} \max_{f\in \Fcal_t^{\dagger}} \left[ \mathbb{E}_{s\sim d^{\pi}_{\widehat{P}_t^\dagger}} f(s) - \sum_{i=1}^N f(s^e_i) / N   \right] $ \Comment{Model-based Planning} 
	%\State Define $\pi_{t+1}(\cdot | s) = \begin{cases} \widehat{\pi}_{t+1}(\cdot | s) & s\in\Kcal_t\\
	%\text{Uniform}(\Acal) & \text{ else}.
	%\end{cases}$, and append to policy cover $\boldpi_{t+1} = \boldpi_t + \{\pi_{t+1}\}$
\EndFor
%\EndFunction
\label{alg:main_alg_bonus}
\end{algorithmic}
\end{algorithm}

We consider the following ground truth model $s' \sim P(\cdot | s,a)$ that consists of a nonlinear dynamics and an additive Gaussian noise:
\begin{align*}
s' = f(s, a) + \epsilon, \epsilon\sim \Ncal(0, \sigma^2 I), 
\end{align*} where $f$ is an unknown nonlinear function. The noise level $\sigma$ is known to the learner. 

Let us assume calibrated model in the following sense. At iteration $t$, learner executes the current policy $\pi_t$ to generate a trajectory $\{s_0, a_0,s_{1}, \dots, s_{H}\}$, which we aggregate it to the replay buffer $\Dcal$. The learner then use the tripls $(s,a,s')$ in the replay buffer $\Dcal$ to train a model $\mu_t(s,a)$, and its uncertainty model $b_t(s,a)$. The model is calibrated if the following is true (in high probability):
\begin{align*}
\left\lvert f(s,a) - \mu_t(s,a) \right\rvert \leq \beta_t b_t(s,a), \forall s,a.
\end{align*}where $\beta_t$ is some parameter. 

\begin{remark}
For KNRs where $f(s,a) = W^\star\phi(s,a)$ with $\phi(s,a)\in\mathbb{R}^d$, we can the uncertainty quantity as $b_t(s,a) := \beta \sqrt{ \phi(s,a)^{\top} \widehat\Sigma_t^{-1} \phi(s,a)}$. For Gaussian process, we have $\mu_t$ being the mean of the GP and $b_t$ being the standard deviation of the GP. In practice, for model ensemble, we could use the standard deviation of the outputs of the models as bonus, which is what we will use in practice
\end{remark}

Given any function $f(s)\in [0,1]$, denote $\widetilde{f}_t$ as $\widetilde{f}_t(s) := f(s)  - \sum_{a\in\Acal} b_t(s,a)$ (\wen{note the sum over $a$ in the reward bonus part, which is important}). Denote $\widetilde{F}_t = \{ \widetilde{f}_t: f \in \Fcal \}$.  Recall $\Fcal$ contains the ground truth cost $c$.


In each model-based planning phase, we perform model-based optimization on the following objective:
\begin{align*}
\pi_{t+1} = \argmin_{\pi\in \Pi} \max_{{f} \in \widetilde{F}_n} \left[ \mathbb{E}_{s \sim d^{\pi}_{\widehat{P}_t} } f(s)  - \sum_{i=1}^N f({s}^e_i) / N  \right].
\end{align*}
%\wen{this is the difference from the absorbing idea: here it's hard to minimize this min-max objective, as $\widehat{P}_t$ could be widely different from $P$;}

\begin{align*}
\max_{{f} \in \widetilde{F}_t} \left[ \mathbb{E}_{s \sim d^{\pi}_{\widehat{P}_t} } f(s)  - \sum_{i=1}^N f({s}^e_i) / N  \right]  & = \max_{{f} \in \widetilde{F}_n} \left[ \mathbb{E}_{s \sim d^{\pi}_{\widehat{P}_t} } f(s)  -   \EE_{s\sim d^{\pi^e}_{\widehat{P}_t}} f(s) +   \EE_{s\sim d^{\pi^e}_{\widehat{P}_t}} f(s)-  \sum_{i=1}^N f({s}^e_i) / N  \right] \\
& \leq  \max_{{f} \in \widetilde{F}_t}\left[ \mathbb{E}_{s \sim d^{\pi}_{\widehat{P}_t} } f(s)  -   \EE_{s\sim d^{\pi^e}_{\widehat{P}_t}} f(s)   \right] + \max_{f\in \widetilde{F}_n } \left[  \EE_{s\sim d^{\pi^e}_{\widehat{P}_t}} f(s)-  \sum_{i=1}^N f({s}^e_i) / N  \right] \\
& \leq  \max_{{f} \in \widetilde{F}_t}\left[ \mathbb{E}_{s \sim d^{\pi}_{\widehat{P}_t} } f(s)  -   \EE_{s\sim d^{\pi^e}_{\widehat{P}_t}} f(s)   \right] + \epsilon_{stats}
\end{align*} where in the last inequality we use the fact that for any $f$, we can set the size of the bonus such that we have optimism for any policy $\pi$:
\begin{align*}
%V^{\pi}_{\widehat{P}_t; \widetilde{f}} \leq V^{\pi}_{P; f} ,
\EE_{s\sim d^{\pi}_{\widehat{P}_t}} \widetilde{f}(s) \leq \EE_{s\sim d^{\pi}} f(s).
\end{align*} The $\epsilon_{stats}$ is the finite sample error from ${s}^e_i$ (i.e., $\epsilon_{stats} = 1/\sqrt{N}$) (See \pref{lem:optimism} in Appendix for proof). 





Hence, for $\pi_{t+1}$, we must have:
\begin{align*}
\max_{{f} \in \widetilde{F}_t} \left[ \mathbb{E}_{s \sim d^{\pi_{t+1}}_{\widehat{P}_t} } f(s)  - \sum_{i=1}^N f({s}^e_i) / N  \right] &  \leq \max_{{f} \in \widetilde{F}_t} \left[ \mathbb{E}_{s \sim d^{\pi^e}_{\widehat{P}_t} } f(s)  - \sum_{i=1}^N f({s}^e_i) / N  \right] \\
& \leq \max_{{f} \in \widetilde{F}_t}\left[ \mathbb{E}_{s \sim d^{\pi^e}_{\widehat{P}_t} } f(s)  -   \EE_{s\sim d^{\pi^e}_{\widehat{P}_t}} f(s)   \right] + \epsilon_{stats} = \epsilon_{stats}.
\end{align*}
Note that $\widetilde{F}_t$ contains $\widetilde{c}_t$, we must have:
\begin{align*}
V^{\pi_{t+1}}_{\widehat{P}_t; \widetilde{c}_t} \lesssim V^{\pi^e}_{P; c} + 2\epsilon_{stats}.
\end{align*} where notation wise we denote $V^{\pi}_{{P}; f}$ as the expected total cost (across $H$ steps) of $\pi$ under transition $P$ and cost function $f$.


This means that the regret in episode $t$ can be characterized as follows:
\begin{align*}
V^{\pi_{t+1}}_{P; c} - V^{\pi^e}_{P; c} & \leq V^{\pi_{t+1}}_{P; c} - V^{\pi_{t+1}}_{\widehat{P}_t;\widetilde{c}_t} + 2 \epsilon_{stats} \\
& =  \EE_{s,a\sim d^{\pi_{t+1}}} \left[ \left\lvert \widetilde{c}_t(s) - c(s) \right\rvert   + H \left\| \widehat{P}_t(\cdot | s,a) - P(\cdot | s,a)  \right\|_1   \right]  +  2 \epsilon_{stat} \\
& \leq \EE_{s,a\sim d^{\pi_{t+1}}} \left[ H \sum_{a\in\Acal} b_t(s,a)   + H  \left\| \widehat{P}_t(\cdot | s,a) - P(\cdot | s,a)  \right\|_1   \right]  +  2 \epsilon_{stat} \\ 
& \leq \EE_{s,a\sim d^{\pi_{t+1}}} \left[ H \sum_{a\in\Acal} b_t(s,a)   + H  b_t(s,a)  \right]  +  2 \epsilon_{stat}\\
& \leq \EE_{s,a\sim d^{\pi_{t+1}}} \left[ H \sum_{a\in\Acal} b_t(s,a)   + H \sum_{a\in\Acal} b_t(s,a)  \right]  +  2 \epsilon_{stat} \\
& \lesssim 2 H \EE_{s \sim d^{\pi_{t+1}}} \left[ \sum_{a\in\Acal } b_t(s,a)   \right] +  2 \epsilon_{stat} \\
& \lesssim H A \EE_{s,a\sim d^{\pi_{t+1}}} b_t(s,a) + 2\epsilon_{stat}
\end{align*}


\wen{finally, we need another assumption that $\sum_{t=1}^T \sum_t b_t(s_h,a_h) = o(T)$, i.e., the information gain grows at most sublinearly. We then give several examples: KNRs and GPs}



\subsection{Is Exploration Necessary in ILFO?}

Note that classic Imitation Learning approaches, e.g., Behavior cloning in offline IL, DAgger in interactive IL, do not require to perform any level of exploration as they simply convert IL into supervised learning (BC converts IL to one SL problem, while DAgger converts it to a sequence of SL problems). However, in ILFO setting, since we do not have experts' action information, converting ILFO to SL is less straightforward. Instead, our algorithm uses bonus and applies the principle of optimism in the face of uncertainty to perform exploration. The key question here is that \emph{in ILFO, is exploration necessary?} We show below that indeed, exploration is necessary in ILFO, in the sense that ILFO is at least as hard as solving a Multi-armed Bandit problem which we know requires exploration and is fundamentally harder than SL. 

Consider a Multi-arm bandit problem with $A$ many actions $\{a_i\}_{i=1}^A$. Each action's ground truth reward $r_i \sim \Ncal(\mu_i, 1)$ is from a Gaussian distribution with mean $\mu_i$ and variance $1$. Without loss of generality, we assume $a_1$ is the optimal arm, i.e., $\mu_1 > \mu_i$ for $i\neq 1$. We convert this MAB instance into the MDP setting that we considered in this work. 
Specifically we set $H = 2$, we have a fixed initial state $s_0$, at $s_0$ we have $A$ many actions. For the one step transition, we have $P( \cdot | s_0, a_i ) = \Ncal(\mu_i, 1)$, i.e., $f(s_0, a_i) = \mu_i$. Here we denote the optimal expert policy $\pi^e$ as $\pi^e(s_0) = a_1$, i.e., expert policy picks the optimal arm in the MAB instance. Hence, when executing $\pi^e$ in this MAB, we note that the state $s_1$ generated from $\pi^e$ is simply the stochastic reward of $a_1$ in the original MAB instance. Assume that we have observed infinitely many such $s_1$ from the expert policy $\pi^e$ (n our algorithm, we have infinitely many expert's state, i.e., $N\to\infty$), this is equivalent to revealing the optimal arm's mean reward $\mu_1$ to the learner a priori.  Hence solving the ILFO problem on this MDP is equivalent to solving the original MAB instance with one more additional information that the optimal arm's mean reward is $\mu_1$.  The following statement indicates that for MAB in general, given the optimal arm's mean reward does not help. 

\begin{theorem}Consider solving Gaussian MAB with an additional information that the optimal arm's mean reward is $\mu$ (i.e., $\mu$ is known but the identity of the best arm is unknown). For any algorithm, there exists a MAB instance with number of arms $K \geq 4$, such that the expected regret is still $\Omega(\sqrt{AT})$, i.e., the additional information does not help improving the worst-case regret bound. 
\label{thm:MAB_lower_bound}
\end{theorem}

Combing the reduction from MAB  with the known optimal arm's mean reward (but not the identity of the optimal arm) to ILFO, and the above theorem, we know that solving ILFO is at least as hard as solving the MAB problem with the known optimal arm's mean reward which itself occurs the same worst case $\sqrt{AT}$ regret bound as the one in the classic MAB setting. The above also shows that in ILFO setting, a polynomially dependency on the number of actions is not avoidable in worst case. 










\iffalse
$\Mhatt, \Mt$ represent the sample based approximation of the known MDP and the true known MDP respectively. Let $\piht, \pihst, \pist$ represent respectively the policy outputted by a planning algorithm on the model-based MDP $\Mhatt$, optimal policy according to $\Mhatt,\Mt$, and $\pie$ is the expert policy. \iffalse We seek to bound:
\begin{align*}
    J(\pie,\M)-J(\piht,\M)&=J(\pie,\M)-J(\pie,\Mt)\\
    &+J(\pie,\Mt)-J(\pist,\Mt)\qquad\qquad(\leq 0)\\
    &+J(\pist,\Mt)-J(\pist,\Mhatt)\qquad\qquad(\text{model error})\\
    &+J(\pist,\Mhatt)-J(\pihst,\Mhatt)\qquad\qquad(\leq 0)\\
    &+J(\pist,\Mhatt)-J(\piht,\Mhatt)\qquad\qquad(\text{Optimization error})\\
    &+J(\piht,\Mhatt)-J(\piht,\Mt)\qquad\qquad(\text{model error})\\
    &+J(\piht,\Mt)-J(\piht,\M)\qquad\qquad(\leq 0).
\end{align*}
\fi


Denote $\Kcal$ as the known state-action set. 
We can define $\pi^e_t$ as the expert policy under $\Mcal_t$, and this gives a $d^{\pi^e_t}_{\Mcal_t}$. Now let us say that we find a policy $\hat{\pi}_t$ such that $\| d^{\hat\pi_t}_{\Mcal_t} -d^{\pi^e_t}_{\Mcal_t}  \|_1$ (via the use of $\widehat{\Mcal}_t$) is tiny. 

Let's say that $\sum_{s,a\not\in\Kcal} d^{\pi^e_t}_{\Mcal_t} = \delta$ is small. This means that $\sum_{s,a\not\in\Kcal} d^{\pi^e}_{\Mcal} = \delta * (1-\gamma)$ is small as well. This should allow us to terminate. 

On the other case,$\sum_{s,a\not\in\Kcal} d^{\pi^e_t}_{\Mcal_t} = \delta$ is big, that means that $\sum_{s,a\not\in\Kcal} d^{\hat\pi_t}_{\Mcal} = \delta$ is kinda big as well. Here we need to argue that we make progress on the elliptical potential. 

Consider the Kernel linear MDP setting, with $\Sigma^{k+1}$ the policy cover of the expert policy with $\Mcal^{k+1}$ (i.e. the $k+1^{st}$ known MDP), and $\Sigma^{k}_{pc} = \frac{1}{k+1}\sum_{l=1}^{k+1}\Sigma_l$. Suppose, we declare an unknown state if $\phi_s^\top (\Sigma^{k}_{pc})^{-1}\phi_s\geq \beta $. Then, it follows that:$$tr((\Sigma^{k}_{pc})^{-1}\Sigma^{k+1})\geq \beta \mathbb{E}_{(s,a)\sim d^{\pi_e}_{t+1}}[\mathbb{I}(s\not\in K^{t+1})].$$ However, what is the potential function? 

Here, we explicitly do not have a value function, though, we are free to choose reward functions for both the actual MDP $\Mcal$ and for $\Mcal^{t+1}$ (not sure if this makes sense). Alternatively, we can consider the state-visitation distributions and say that $$d^{e}\geq d^e_{t+1}-\mathbb{E}_{s\sim d^e}[\mathbb{I}(s\not\in K^{t+1})],$$ which can be used to derive the elliptical potential function argument. 
\fi


==> macros.tex <==
%!TEX root = corruption_main.tex
\newcommand{\LR}{\mathrm{LR}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\pl}{(1)}
\newcommand{\kl}{_{k,\ell}}
\newcommand{\klh}{_{k,\ell;h}}
\newcommand{\klpr}{_{k,\ell'}}
\newcommand{\klprh}{_{k,\ell';h}}
\numberwithin{equation}{section}


\newcommand{\wkl}{\weight\kl}
\newcommand{\wklh}{\weight\klh}
\newcommand{\nbar}{\overline{n}}
\newcommand{\nbark}{\nbar_k}
\newcommand{\eventproblelst}{\mathcal{E}^{\mathrm{lead},\le\lst}}
\newcommand{\eventprobl}{\mathcal{E}^{\mathrm{lead},\ell}}

\newcommand{\eventvalconc}{\mathcal{E}^{\mathrm{val,conc}}}
\newcommand{\eventprobconc}{\mathcal{E}^{\mathrm{prb,conc}}}
\newcommand{\xaxpr}{(x,a,x')}
\newcommand{\goodeps}{\mathcal{K}_{\mathrm{good}}}
\newcommand{\advrange}{\adv^{\mathrm{range}}}
\newcommand{\corrupt}{\mathbf{C}}
\newcommand{\Err}{\mathrm{Err}}



\newcommand{\Klst}{\lst}
\newcommand{\jh}{_{j;h}}
\newcommand{\jhpl}{_{j;h+1}}
\newcommand{\eventsub}{\calE^{\mathrm{subsmp}}}
\newcommand{\klsthpl}{_{k,\lst;h+1}}
\newcommand{\hpl}{_{h+1}}
\newcommand{\klhpltwo}{_{k,l;h+2}}
\newcommand{\xpr}{x'}
\newcommand{\klihpl}{_{k,\ell,i;h+1}}
\newcommand{\lmaxj}{\lmax_j}
\newcommand{\alphali}{\alpha_{\ell,i}}
\newcommand{\iset}{\left\{\mathrm{sb},\mathrm{gl}\right\}}
\newcommand{\corruptk}{\corrupt_k}
\newcommand{\didcorruptk}{\didcorrupt_k}
\newcommand{\eventconc}{\mathcal{E}^{\mathrm{conc}}}
 \newcommand{\klihpr}{_{k,\ell,i;h'}}

\newcommand{\boundlead}{\bound^{\mathrm{lead}}}
\newcommand{\boundcross}{\bound^{\mathrm{cross}}}
\newcommand{\boundtotal}{\bound^{\mathrm{total}}}
\newcommand{\xau}{(x,a;u)}
\newcommand{\bound}{\mathbf{B}}
\newcommand{\delv}{\Delta \vup}

\newcommand{\Errlead}{\Err^{\mathrm{val}}}
\newcommand{\klglb}{_{k,\ell,\mathrm{gl}}}
\newcommand{\klsub}{_{k,\ell,\mathrm{sb}}}
\newcommand{\klelst}{_{k,\le \lst}}
		\newcommand{\klst}{_{k,\lst}}

	\newcommand{\Pikl}{\Pi_{k}^{\ell}}
	\newcommand{\Piklelst}{\Pi_{k}^{\le\lst}}
\newcommand{\Pik}{\Pi_k}
\newcommand{\kli}{_{k,l,i}}
\newcommand{\klpl}{_{k,\ell+1}}
\newcommand{\klminh}{_{k,\ell-1;h}}
\newcommand{\piucb}[1]{\boldpi^{\mathrm{ucb},#1}}
\newcommand{\boldlk}{\boldl_k}
\newcommand{\Finite}[1]{\left[#1\right]_{<\infty}}
\newcommand{\nk}{n_k}
\newcommand{\nkl}{n_{k,\ell}}
\newcommand{\robustLfactor}{\Lfactor^{\mathrm{rbst}}}
\newcommand{\klih}{_{k,\ell,i;h}}
\newcommand{\Index}{\mathcal{I}}
		\newcommand{\klhpl}{_{k,\ell,h+1}}
\newcommand{\lfin}{\boldl^{\mathrm{fin}}}
\newcommand{\lmax}{\boldl^{\mathrm{max}}}
\newcommand{\klsth}{_{k,\lst;h}}
	\newcommand{\lst}{\ell_{\star}}
\newcommand{\Regret}{\mathrm{Regret}}

\newcommand{\pigreedboldl}{\pi^{\mathrm{ucb},\,(\boldl)}}
	\newcommand{\pigreedboldlk}{\pi^{\mathrm{ucb},\,(\boldl)}_k}
	\newcommand{\pigreedboldlkk}{\pi^{\mathrm{ucb},\,(\boldl_k)}_k}
\newcommand{\distlayer}{\mu_{\mathrm{layer}}}
 
\newcommand{\boldpik}{\boldsymbol{\pi}_k}
\newcommand{\boldpil}{\boldsymbol{\pi}^{\ell}}
\newcommand{\boldpilk}{\boldsymbol{\pi}^{\ell}_k}

\newcommand{\boldpilel}{\boldsymbol{\pi}^{\le\ell}}
\newcommand{\boldpilelst}{\boldsymbol{\pi}^{\le\lst}}


\newcommand{\boldpilelk}{\boldsymbol{\pi}^{\le\ell}_k}
\newcommand{\boldpilelstk}{\boldsymbol{\pi}^{\le\lst}_k}
\newcommand{\ellset}{\mathscr{L}}
\newcommand{\ellsetl}{\ellset_{\ell}}
\newcommand{\xkhakh}{(\matx\kh,\mata\kh)}
\newcommand{\xjhajh}{(\matx\jh,\mata\jh)}

\newcommand{\klplh}{_{k,\ell+1;h}}
\newcommand{\oplustau}{\oplus_{\tau}}
\newcommand{\oplush}{\oplus_{h}}
\newcommand{\oplushbar}{\oplus_{\hbar}}
\newcommand{\vsthpl}{\vst_{h+1}}
\newcommand{\xah}{(x,a,h)}
\newcommand{\gap}{\mathrm{gap}}
\newcommand{\gapmin}{\gap_{\min}}
\newcommand{\clip}[2]{\operatorname{clip}\left[#2|#1\right]}
\newcommand{\clipmid}[2]{\operatorname{clip}\left[#2\mid\,#1\right]}

\newcommand{\cliptil}[2]{\widetilde{\operatorname{clip}}\left[#2|#1\right]}

\newcommand{\advlucbhalfclip}{\dot{\adv}^{\mathrm{lucb}}}
 \newcommand{\advhalfclip}{\dot{\adv}}
 \newcommand{\phatk}{\phat_k}
\newcommand{\rhatk}{\rhat_k}
 \newcommand{\advlucbfullclip}{\ddot{\adv}^{\mathrm{lucb}}}
 \newcommand{\advfullclip}{\ddot{\adv}}
\newcommand{\gaph}{\mathrm{gap}_h}
\newcommand{\epsclip}{\epsilon_\mathrm{clip}}
\newcommand{\vsth}{\vst_h}
\newcommand{\mup}{\overline{\calM}}
\newcommand{\mlow}{\underline{\calM}}
\newcommand{\mlowk}{\mlow_k}
\newcommand{\mupk}{\mup_k}
\newcommand{\vupk}{\vup_k}
\newcommand{\vlowk}{\vlow_k}
\newcommand{\qlowk}{\qlow_k}
\newcommand{\qupk}{\qup_k}
\newcommand{\pigreedk}{\pigreed_k}
\newcommand{\ofx}{(x)}
\newcommand{\ofxh}{(x_h)}
\newcommand{\pisth}{\pist_h}
\newcommand{\xhah}{(x_h,a_h)}


\renewcommand{\ast}{a^\star}
\newcommand{\xast}{(x,\ast)}
\newcommand{\qsth}{\qst_h}
\newcommand{\bolda}{\mathbf{a}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\activeset}{\mathscr{A}}
\newcommand{\activesetk}{\activeset_k}
\newcommand{\tuple}{\mathscr{T}}
\newcommand{\tuplek}{\tuple_k}
\newcommand{\Kpl}{K^{\pl}}
\newcommand{\matz}{\mathbf{z}}
\newcommand{\matxpl}{\matx^{\pl}}
\newcommand{\matypl}{\maty^{\pl}}
\newcommand{\calEtil}{\widetilde{\mathcal{E}}}
\newcommand{\kclass}{\mathscr{K}}
\newcommand{\lossid}[1]{\mathcal{L}_{\mathrm{id},#1}}

\newcommand{\advlucb}{\adv^{\mathrm{lucb}}}
\newcommand{\advlowgreed}{\advlow^{\mathrm{lcb}}}


\newcommand{\boldl}{\boldsymbol{\ell}}


\newcommand{\valf}{\boldsymbol{V}}
\newcommand{\vst}{\valf^{\star}}
\newcommand{\qst}{\qf^{\star}}
\newcommand{\pist}{\pi^{\star}}


\newcommand{\qf}{\boldsymbol{Q}}
\newcommand{\vup}{\bar{\valf}}
\newcommand{\qup}{\bar{\qf}}
\newcommand{\qlow}{\makelow{\qf}}
\newcommand{\vlow}{\makelow{\valf}}

\newcommand{\qcirc}{\mathring{\qf}}
\newcommand{\vcirc}{\mathring{\valf}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\adv}{\mathbf{A}}

\newcommand{\advcirc}{\mathring{\adv}}

\newcommand{\occ}{\boldsymbol{\omega}}

\newcommand{\phat}{\widehat{p}}
\newcommand{\rhat}{\widehat{r}}

\newcommand{\rhatkhl}{\rhat_{k,h,\ell}}
\newcommand{\khl}{_{k;h;l}}
\newcommand{\khbar}{_{k;\hbar}}

\newcommand{\khboldl}{_{k;h,\boldl}}

\newcommand{\khlpr}{_{k,h,l'}}
\newcommand{\khpl}{_{k;h+1}}
\newcommand{\khpr}{_{k;h'}}

\newcommand{\khlh}{_{k,h,\boldl_h}}
\newcommand{\xa}{(x,a)}


\newcommand{\makelow}[1]{\mkern2mu\underline{\mkern-2mu#1\mkern-4mu}\mkern4mu }


\newcommand{\bonus}{\boldsymbol{b}}
\newcommand{\bonuskhl}{\bonus_{k,h,\ell}}
\newcommand{\bonusbar}{\overline{\bonus}}
\newcommand{\bonuscirc}{\mathring{\bonus}}

\newcommand{\nkhl}{n_{k,h,\ell}}
\newcommand{\Lfactor}{\mathbf{L}}
\newcommand{\Lcorrupt}{\mathbf{L}_{\mathrm{crpt}}}

\newcommand{\cbon}{c_{\bonus}}
\renewcommand{\hbar}{\tau}
\newcommand{\hboldbar}{\overline{\boldsymbol{\tau}}}


\renewcommand{\ast}{a^\star}

\newcommand{\kh}{_{k;h}}
\newcommand{\boldpi}{\boldsymbol{\pi}}
\newcommand{\pigreed}{\pi^{\mathrm{ucb}}}
\newcommand{\piexp}{\pi^{\mathrm{exp}}}
\newcommand{\pimix}{\pi}
\newcommand{\pilcb}{\pi^{\mathrm{lcb}}}
\newcommand{\calMlow}{\makelow{\calM}}
\newcommand{\advlow}{\makelow{\adv}}
\newcommand{\bonuslow}{\makelow{\bonus}\,}


\newcommand{\weight}{\boldsymbol{\omega}}
\newcommand{\weighthbar}{\weight^{\hbar}}

\newcommand{\khhbar}{_{k,h;\hbar}}
\newcommand{\khhboldbar}{_{k,h;\hboldbar}}
\newcommand{\dens}{\rho}
\renewcommand{\colon}{{\,:\,}}
\newcommand{\calM}{\mathcal{M}}

\newcommand{\calMbar}{\overline{\calM}}
\newcommand{\pbar}{\overline{p}}
\newcommand{\rbar}{\overline{r}}

\newcommand{\states}{\mathcal{X}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\outputs}{\mathcal{Y}}
\newcommand{\matx}{\mathbf{x}}
\newcommand{\mata}{\mathbf{a}}

\newcommand{\Gclass}{\mathscr{G}}
\newcommand{\Ust}{U_{\star}}
%\newcommand{\Vst}{V_{\star}}
\newcommand{\sfP}{\mathsf{P}}

\newcommand{\Ast}{A_{\star}}
\newcommand{\Bst}{B_{\star}}
\newcommand{\Kst}{K_{\star}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\Khat}{\widehat{K}}
\newcommand{\matU}{\mathbf{U}}
\newcommand{\matDel}{\boldsymbol{\Delta}}
\newcommand{\Rhat}{\widehat{R}}

\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\ProjK}{\mathrm{Proj}_{\Kst}}
\newcommand{\ProjKzero}{\mathrm{Proj}_{\mathbf{0} \oplus \Kst}}
\newcommand{\veczero}{\mathbf{0}}

\newcommand{\Stief}{\mathrm{Stief}}
\newcommand{\nablabar}{\overline{\nabla}}
\newcommand{\nablacheck}{\check{\nabla}}
\newcommand{\fcheck}{\check{f}}
\newcommand{\Gcheck}{\check{G}}

\newcommand{\calK}{\mathcal{K}}
\newcommand{\calE}{\mathcal{E}}

\newcommand{\Rcheck}{\check{R}}

\newcommand{\xbar}{\overline{x}}
\newcommand{\xcheck}{\check{x}}


%comments

%ceiling
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%theorems
{
 \theoremstyle{plain}
      \newtheorem{asm}{Assumption}
}
\newtheorem{nono-theorem}{Theorem}[]
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
%\theoremstyle{remark}
%\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}

\newtheorem{prop}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{example}{Example}[section]
\newtheorem{exc}{Exercise}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{obs}{Observation}[section]


%probability
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

\newcommand{\Law}{\mathrm{Law}}
\newcommand{\Leb}{\mathrm{Lebesgue}}

\newcommand{\unifsim}{\overset{\mathrm{unif}}{\sim}}
\newcommand{\iidsim}{\overset{\mathrm{i.i.d.}}{\sim}}
\newcommand{\probto}{\overset{\mathrm{prob}}{\to}}
\newcommand{\ltwoto}{\overset{L_2}{\to}}

\newcommand{\info}{\mathbf{i}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\Ent}{\mathrm{Ent}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\rmd}{\mathrm{d}}

%math operators
\newcommand{\median}{\mathrm{Median}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\im}{\mathrm{im }}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\spec}{\mathrm{spec}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\sign}{\mathrm{sign\ }}
\newcommand{\abs}{\mathrm{abs\ }}

%norms
\newcommand{\op}{\mathrm{op}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\dist}{\mathrm{dist}}

% logical
\renewcommand{\implies}{\text{ implies }}
\renewcommand{\iff}{\text{ iff }}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\matbeta}{\boldsymbol{\beta}}
\newcommand{\mattheta}{\boldsymbol{\theta}}

\newcommand{\betast}{\matbeta^*}
\newcommand{\betahat}{\widehat{\matbeta}}

\newcommand{\thetast}{\mattheta^*}
\newcommand{\thetahat}{\widehat{\mattheta}}
\newcommand{\supp}{\mathrm{supp}}


\newcommand{\matw}{\mathbf{w}}
\newcommand{\maty}{\mathbf{y}}


%Number Spaces
\renewcommand{\Im}{\mathfrak{Im }}
\renewcommand{\Re}{\mathfrak{Re }}
\newcommand{\N}{\mathbb{Z}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\Q}{\mathbb{Q}}

%Vector Spaces
\newcommand{\PD}{\mathbb{S}_{++}^d}
\newcommand{\sphered}{\mathcal{S}^{d-1}}




% Asymptotics
\DeclareMathOperator{\BigOm}{\mathcal{O}}
\newcommand{\BigOh}[1]{\BigOm\left({#1}\right)}
\DeclareMathOperator{\BigOmtil}{\widetilde{\mathcal{O}}}
\newcommand{\BigOhTil}[1]{\BigOmtil\left({#1}\right)}
\DeclareMathOperator{\BigTm}{\Theta}
\newcommand{\BigTheta}[1]{\BigTm\left({#1}\right)}
\DeclareMathOperator{\BigWm}{\Omega}
\newcommand{\BigThetaTil}[1]{\widetilde{\BigTm}\left({#1}\right)}
\newcommand{\BigOmega}[1]{\BigWm\left({#1}\right)}
\DeclareMathOperator{\LittleOm}{\mathrm{o}}
\newcommand{\LittleOh}[1]{\LittleOm\left({#1}\right)}
\DeclareMathOperator{\LittleWm}{\omega}
\newcommand{\LittleOmega}[1]{\LittleWm\left({#1}\right)}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\logdet}{log\,det}

\newcommand{\Rsimple}{\mathcal{R}_{\mathrm{simp}}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\actst}{a_*}
\newcommand{\acthat}{\widehat{a}}


\newcommand{\lasso}{\mathsf{lasso}}
\newcommand{\four}{\mathscr{F}}
\newcommand{\LS}{\mathsf{LS}}
\newcommand{\Alg}{\mathsf{Alg}}


\newcommand{\vi}{\matv^{(i)}}

% Complexity Classes
\newcommand{\SAT}{\mathit{SAT}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\coNP}{\co{NP}}
\newcommand{\co}[1]{\mathbf{co#1}}

%%%%%%PG%%%%%%%
\newcommand{\dboldpi}{d_{\boldpi}}
\newcommand{\dpi}{d_{\pi}}
\newcommand{\sink}{s^{\dagger}}
\newcommand{\abmdp}{\calM^{\dagger}}


%%%%% Akshay's macros %%%%%
\newcommand{\epsstat}{\varepsilon_{\textrm{stat}}}
\newcommand{\bellman}{\mathcal{T}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\qhat}{\widehat{Q}}
\newcommand{\vhat}{\widehat{V}}
\newcommand{\aphi}{A\circ\phi}
\newcommand{\supi}{^{(i)}}
\newcommand{\calV}{\mathcal{V}}
%\newcommand{\xhah}{(x_h,a_h)}
